ACE: Abstract Consensus Encapsulation for Liveness Boosting of State Machine Replication

With the emergence of cross-organization attack-prone byzantine fault-tolerant (BFT) systems, so-called Blockchains, providing asynchronous state machine replication (SMR) solutions is no longer a theoretical concern. This paper introduces ACE: a general framework for the software design of fault-tolerant SMR systems. We first propose a new leader-based-view (LBV) abstraction that encapsulates the core properties provided by each view in a partially synchronous consensus algorithm, designed according to the leader-based view-by-view paradigm (e.g., PBFT and Paxos). Then, we compose several LBV instances in a non-trivial way in order to boost asynchronous liveness of existing SMR solutions. ACE is model agnostic - it abstracts away any model assumptions that consensus protocols may have, e.g., the ratio and types of faulty parties. For example, when the LBV abstraction is instantiated with a partially synchronous consensus algorithm designed to tolerate crash failures, e.g., Paxos or Raft, ACE yields an asynchronous SMR for $n = 2f+1$ parties. However, if the LBV abstraction is instantiated with a byzantine protocol like PBFT or HotStuff, then ACE yields an asynchronous byzantine SMR for $n = 3f+1$ parties. To demonstrate the power of ACE, we implement it in C++, instantiate the LBV abstraction with a view implementation of HotStuff -- a state of the art partially synchronous byzantine agreement protocol -- and compare it with the base HotStuff implementation under different adversarial scenarios. Our evaluation shows that while ACE is outperformed by HotStuff in the optimistic, synchronous, failure-free case, ACE has absolute superiority during network asynchrony and attacks.

==> DistributedLedger.tex <==
\section{Optimistic Efficient replicated ledger}

% Note that state machine replication with weak Termination is
% a weaker problem than atomic broadcast.
% In particular, it does not require a state transfer.
% However, it is strong enough for practical purposes since a read
% operation has anyway to communicate with a quorum of the parties due
% to possible failures.


In this section we extend our optimistic single-shot Agreement
protocol into an optimistic replicated ledger.
For our replicated ledger we choose the slot by slot approach, meaning
that parties do not move to the next slot before a decision was made
on the previous one. \sasha{TODO: give motivation for this choice -
either here or before. Also, maybe it should be a property of the
problem definition.}
In best case scenario (synchrony and an honest leader), all parties
move together from one slot to the next.
However, in general, it is possible for some honest parties to move
forward, while others are stuck in previous slots.
To deal with this issues, we slightly strengthen the properties
required by the LBV primitive and define an additional long-lived
primitive in Section~\ref{sub:SMRprimitives}.
In Section~\ref{sub:SMRptorocol}, we present our optimistic replicated
ledger protocol.


% The pseudocode for the general optimistic efficient distributed
% ledger algorithm appears in Algorithm~\ref{alg:optomisticDL}.
% In best case scenario (synchrony and an honest leader), all parties
% move together from one slot to the next.
% However, in general, it is possible for some honest parties to move
% forward, while others are stuck in previous slots because they did not
% decide.
% To deal with this issues, we use the provability properties defined in
% the previous section, to honest parties convince parties to
% move forward.
% Note that sending proves requires a quadratic all to all
% communication.
% Therefore, in order to be able to satisfy optimism honest parties send
% such proofs only before they face parts in the algorithm that require
% participation of all good parties for Termination i.e., tryPasimistic
% procedure and \emph{view-change} primitive.
% Since the complexity of these parts is at least quadratic any why,
% sending forward proofs do not impact the overall complexity.
% \sasha{TODO: describe the protocol.}


\subsection{Primitives for replicated ledger}

Recall that by Halting, all honest parties in a given slot eventually
halt.
But by Noticeable Termination, some honest parties may never decide,
and thus never move forward to the next slot.
Therefore, slow parties must be able to learn that enough honest
parties decided and thus the Termination property is satisfied and
they can safely move forward.
Similarly, parties stuck in slow slots might advance their view, and
thus even if they eventually jump forward to the next slot, other
parties need to jump forward to their view.
To this end, we need to slightly strengthen the properties
required by the LBV primitive and define an additional cross-slot and
cross-view primitive we call \emph{coordinator}.


%  honest parties that do move must be able to convince slow
% ones that enough parties have decided and it is safe to move forward.
% To this end, in order to be able to generalize the optimistic (single
% shoot) Agreement into an optimistic distributed ledger, we need to
% slightly strengthen the properties required by the primitives we use
% in order to allow parties to prove their outputs.
% Note that in case of crash failures we get this for free, while in the
% byzantine failure case, some cryptography is required. 

\paragraph{Extended LBV}

We now define an extended LBV we denote by \emph{exLBV}.
In addition to to state and value, the \emph{learn} API of eLBV 
returns a Boolean \emph{done}, which intuitively indicates
that enough honest parties decided.
The Propose-Termination, Learn-Termination, Validity, and
Agreement properties are the same as in LBV.
The only difference is in the Completeness property and the existence
of additional Causality property:

\begin{itemize}
  
  \item  \textbf{exCompleteness:} For every instance, if a {propose}
  invocation by an honest leader returns, then no {learn}
  invocation by honest party returns $done = false$.
  
  \item For every instance, if a {propose}
  invocation by an honest leader returns, then (1) at least $f+1$
  approve invocations by honest parties return $v \neq \bot$ and (2)
  no {learn} invocation by an honest party returns {value} $v = \bot$.
  
  \item  \textbf{exCausality:} For every instance, if a {learn}
  invocation by an honest party returns $done = true$, then no
  {learn} invocation by honest party returns $v = \bot$.
  
\end{itemize}







\input{DistributedLedgerAlg.tex}

==> DistributedLedgerAlg.tex <==
\begin{algorithm}
\caption{Optimistic SMR: protocol for party $p_i$.} 
\begin{algorithmic}[1]
\small

\State \textbf{Local variables:}
\State \hspace*{0.4cm} \emph{state}; \emph{log}; \emph{slot};
\emph{view}; \emph{slotDone}; \emph{viewDone}

\Statex

\Upon{\emph{OpSMR-propose(S)}}

\State $state \gets S$; $slot \gets 1$; $view \gets 1$

% \While {true}
\State  $try()$


% \EndWhile

\EndUpon

\Statex

\Procedure{try()}{}
  
  \State $id \gets \lr{slot,view}$
  \If{\emph{mode}$(view) = $ \textsc{optimistic}}  
	 	
		\State  $\lr{state, value, leader, leaderProof, doneProof} \gets
		tryOptimistic(id, state)$ 
	\Else
	
		\State send ``\textsc{jump-forward}$, slot, \emph{slotDone}, view,
		\emph{viewDone}$'' to all parties 
		\State $\lr{state, value, leader, leaderProof, doneProof} \gets
		tryPasimistic(id, state)$
	\EndIf
	
% 	\State  $\lr{state,value} \gets try(slot, view, state)$
% 	\State invoke $\emph{OpA-propose}(slot, state)$
	
	\If{$doneProof = \bot$ }
		\State send ``\textsc{jump-forward}$, slot, \emph{slotDone}, view,
		\emph{viewDone}$'' to all parties
		\State invoke $\emph{trigger}_{id}()$
		\State $\sigma \gets \emph{trigger-sync}_{id}()$
		\State $\emph{viewDone} \gets \lr{slot,\sigma}$
		\State $\lr{state,value} \gets VC_{id}(state,value)$
% 		\State \emph{increaseView}$(\emph{viewDone})$

		\State $view \gets view + 1$
		\State $try()$
		
	\Else
	
		\State $log[slot].value \gets value$
		\Comment{\textbf{decide} $\lr{slot,value}$}
		\State $\emph{slotDone} \gets \lr{view,leader, leaderProof,
		doneProof}$
		\Comment{completeness proof for \emph{doneVerify}}
% 		\State \emph{increaseSlot}$(\emph{slotDone})$

		\State $slot \gets slot+1$
		\If{\emph{mode}$(view) = $ \textsc{pessimistic}}
		
			\State $view \gets view + 1$
		
		\EndIf
		
		\State $try()$	
	
	\EndIf
	
 	
\EndProcedure

\Statex

% \Procedure{increaseSlot}{\emph{slotDone}}
% 
% 	\State $slot \gets slot+1$
% 	\State in crease the view in case of pessimistic mode
% 	\State $try(slot, view)$
% 
% \EndProcedure
% 
% \Statex
% 
% \Procedure{increaseView}{$\sigma$}
% 
% 	\State $view \gets view + 1$
% 	\State $try(slot, view)$
% 
% \EndProcedure
% 
% \Statex


\Receiving{``\textsc{jump-forward}$, slot', \emph{SDone}, view',
		\emph{VDone}$''}
		
	\State \emph{retry} $\gets$ \emph{false}
	\State \emph{slotLeaderID} $\gets \lr{\emph{slot'}-1,
		\emph{SDone}.view}$
	\State \emph{slotDoneID} $\gets \lr{slot'-1, \emph{SDone}.view,
	\emph{SDone}.leader}$
	\State \emph{viewBarrierID} $\gets \lr{\emph{VDone}.slot, view'-1}$		
	\Statex
	\If{\emph{mode}$(\emph{SDone}.view) = $
		\textsc{pessimistic}} 
	
		\If{$\emph{leaderVerify}(slotLeaderID,\emph{SDone}.leader,
		\emph{SDone}.leaderProof) =$ \emph{false}}
		
		
			\State \textbf{return}
		\EndIf
	 
	\EndIf
	
		\If{\emph{mode}$(\emph{SDone}.view) = $
		\textsc{optimistic}} 
	
		\If{\emph{SDone}.leader $\neq$ \emph{getLeader(view)}}
		
		
			\State \textbf{return}
		\EndIf
	 
	\EndIf
	
	\If{$slot' > slot ~\wedge~
	\emph{doneVerify}(slotDoneID, \emph{SDone}.doneProof) =
	\emph{true}$}
	
		\State \emph{retry} $\gets$ \emph{true};~
		$slot \gets slot'$;~
		$\emph{slotDone} \gets \emph{SDone}$
		
		\If{$\emph{SDone}.view \geq
		view ~\wedge~$ \emph{mode}$(\emph{SDone}.view) = $
		\textsc{pessimistic}}
		
			\State $view \gets \emph{SDone}.view + 1$
		
		\EndIf
	
	\EndIf
	
	\If{$view' > view ~\wedge~
	\emph{barrierVerify}(viewBarrierID,
	\emph{VDone}.proof) = \emph{true}$}
	
		\State \emph{retry} $\gets$ \emph{true};~ 
		 $view \gets view'$;~
		$\emph{viewDone} \gets \emph{VDone}$
	
	\EndIf
	
	\If{retry}
	
		\State kill all other processes
		\State $try()$
	
	\EndIf

\EndReceiving




\end{algorithmic}
\label{alg:optomisticDL}
\end{algorithm}


==> OSSagreement.tex <==
\begin{algorithm}
\caption{Optimistic agreement: protocol for party $p_i$.} 
\begin{algorithmic}[1]
% \small

\Upon{\emph{OpA-propose(id, S)}}

\State $state \gets S$ 
\State $view \gets 1$

\While {true}

	\State $id \gets view$
	\If{\emph{mode}$(view) = $ \textsc{optimistic}}  
% 	\Comment{$m > 1$}
	 
		\State  $ \lr{state',value'\textcolor{gray}{,doneProof}} \gets \Call{tryOptimistic}{id, state}$
		
	\Else
	
		\State  $\lr{state',value'\textcolor{gray}{,doneProof}} \gets \Call{tryPessimistic}{id, state}$	
	
	\EndIf
	
	%\State $\lr{state',value' \textcolor{gray}{, doneProof}} \gets learn_{\lr{id, leader}}()$


	\If{$value' = \bot$ }
	
		\State invoke $\emph{trigger}_{id}()$
		
	\Else
	
		\State \textbf{decide} $value'$	
	
	\EndIf
	
	\State \emph{trigger-sync}$_{id}()$	
	
	\State $state \gets state'$
	
	\State $view \gets view+1$ 
	


\EndWhile

\EndUpon

\Statex

  \Procedure{tryOptimistic}{$id, state$}
  
 	\State $leader \gets getLeader(id)$
	\Comment{Local and deterministic}

	\State $timedOut \gets false$

	\If{$leader = p_i$}
	
		\State invoke $propose_{\lr{id,p_i}}(state)$
		\Comment{non-blocking}
	
	\EndIf
	\State  invoke \emph{timer$(id)$}
	\Comment{non-blocking}	

	\State wait until \emph{approve} returns or $timedOut$ is $true$

	%\State $\lr{state',value'\textcolor{gray}{,doneProof}} \gets
	%approve_{\lr{id,leader}}(state)$

	\State $\lr{state',value'\textcolor{gray}{,doneProof}} \gets learn_{\lr{id,leader}}()$
	
	%\State \textbf{return} $\lr{state',value' \textcolor{gray}{, leader,
	%\bot, doneProof}}$
	%\State $\lr{state',value' \textcolor{gray}{, doneProof}} \gets learn_{\lr{id, leader}}()$

	\State \textbf{return} $\lr{state',value'\textcolor{gray}{,doneProof}}$
 	
\EndProcedure

\Statex 

\Upon{\emph{timer$(id)$} returns}

	%\State invoke $abandon_{\lr{id,leader}}()$
	%\Comment{$approve_{\lr{id,leader}}$ immediately returns}
	\State $timedOut \gets true$
	

\EndUpon


\end{algorithmic}
\label{alg:optimisticAgreement}
\end{algorithm}


==> PS.tex <==
\subsubsection{Partial synchrony}
\label{subsec:ES}

\textcolor{red}{TODO: The GST and timeouts must be better defined. Do
we want to use failure detectors or increasing timeouts like in PBFT?}
\ittai{I would prefer GST}


The pseudocode is given in Algorithm~\ref{alg:PS}, and an
illustration appear in Figure~\ref{fig:ESprotocol}.
The function \emph{getLeader} returns leaders in a
deterministic, pre-defined, and known to all order. 
% The only required property is that for every party $p_i$ there are
% infinite number of views in which $p_i$ is returned.
The function \emph{timer(id)} returns after the time parties are
willing to wait before abandoning the \LBP\ with identification $id$
is passed. \DM{this is not enough for liveness. we need all honest parties to
spend enough time in overlap in some view. That is, there must be a period $P$, 
and some view $v$, such that all honest parties and the leader
for the view are in view $v$ during $P$, and $P$ is long enough to execute
leader() without abandon(). Question: Why provide a partially synchronous
solution at all??}




\begin{algorithm}
\caption{Agreement in a partially synchronous environment: protocol
for party $p_i$.} 
\begin{algorithmic}[1]
% \small

\Upon{\emph{ES-propose(S)}}

\State $state \gets S$ 
\State $view \gets 1$

\While {true}

	\State $id \gets view$
	\State $ \lr{state, value\textcolor{gray}{, leader,
	leaderProof, doneProof}} \gets tryOptimistic(id, state)$ 
	\State $\lr{state,value} \gets VC_{id}(state,value)$
	
	\If{$value \neq \bot$ }
	
		\State \textbf{decide} value
	
	\EndIf
	
	\State $view \gets view+1$ 
	


\EndWhile

\EndUpon

\Statex

  \Procedure{tryOptimistic}{$id, state$}
  
 	\State $leader \gets getLeader(id)$
	\Comment{Local and deterministic}
% 	\State $TO \gets getTimeout(view)$
	
	\If{$leader = p_i$}
	
		\State invoke $propose_{\lr{id,p_i}}(state)$
		\Comment{non-blocking}
	
	\EndIf
		
	\State  invoke \emph{timer$(id)$}
	\Comment{non-blocking}	
	\State $\lr{state',value'\textcolor{gray}{,doneProof}} \gets
	approve_{\lr{id,leader}}(state)$
	
% 	\State invoke $approve_{[view,leader]}(state)$
% 	\Comment{non-blocking}
% 	\State  invoke \emph{timer}	
% 	\State wait for $timeout$ or $approve_{[view,leader]}$ to return
% 	$\lr{state',value'}$
% 	\If{$timeout$}
% 	
% 		\State invoke $abandon_{[view,leader]}()$
% 		\Comment{$approve$ immediately returns $\lr{state',value'}$}
% 	\EndIf
	
	\State \textbf{return} $\lr{state',value' \textcolor{gray}{, leader,
	\bot, doneProof}}$
 	
\EndProcedure

\Statex 

\Upon{\emph{timer$(id)$} returns}

	\State invoke $abandon_{\lr{id,leader}}()$
	\Comment{$approve_{\lr{id,leader}}$ immediately returns}
	

\EndUpon


\end{algorithmic}
\label{alg:PS}
\end{algorithm}


\paragraph{Correctness proof.}
We now prove that Algorithm~\ref{alg:PS} implements Agreement with
deterministic termination in the partial synchrony model.
Since Algorithm~\ref{alg:PS} constructs a legal executions of the
\LBP\ and view-change abstractions, the \emph{validity} and
\emph{agreement} properties are trivially satisfied by the
assumptions.
We now prove termination.


\begin{claim}
\label{claim:viewcomplete}

For every $k \geq 1$, all parties eventually complete view $k$. 

\end{claim}

We prove the claim by induction.

\textbf{Base:} We start by proving the claim for $view =1$.
The functions \emph{getLeader} and \emph{getTimeout} are local so no
party can stuck there.
By the LBP-Abandonment property of the \LBP\ and the fact that all
parties invoke abandon after the timeout has expired, we get that
every \emph{approve}$_{[1,leader]}$ operation eventually
returns.
Therefore, all honest parties invoke $VC_{[1]}$, and thus, by the
\emph{VC-termination} property, all $VC$ invocations by honest parties
eventually return.
Hence, all honest parties eventually complete view 1.

\textbf{Step:} Assume that all honest parties complete view $k \geq
1$, we show that all honest parties complete view $k+1$.
By the assumption, all honest parties start view $k+1$.
Thus, the lemma follows by applying the same arguments as in the base
case.


\begin{claim}

All parties in Algorithm~\ref{alg:PS} eventually decide.

\end{claim}

\begin{proof}

By Claim~\ref{claim:viewcomplete} and the properties of
\emph{getLeader}, there is a view $k$ that all honest parties start
after the GST and \emph{getLeader(k)} returns the same honest leader
$p_l$ to all parties.
Therefore, all honest parties invoke \textbf{approve}$_{[k,p_l]}$, and
since it happens after the GST, we get by LBP-Termination, that
$p_l$'s propose invocation returns.
Therefore, by LBP-Completeness, at least $f+1$ honest parties return
$value \neq \bot$.
By claim~\ref{claim:viewcomplete}, all  $VC_{[k]}$ invocations by
honest parties return, and thus by the VC-causality property, all
honest party return $value \neq \bot$.
Therefore, all honest party decide in view $k$.


\end{proof}



==> ProblemDefinition.tex <==
% \subsection{Single-shot Agreement}
% 
% We use the VABA version because this what we need for a distributed
% ledger.
% 
% Maybe merge 3.2 and 3.3 in order to give some intuition for VABA
% definition.

% Halting.

\subsection{Problem Defintion}

In this section we formally define the problems our generic framework
solves in this paper.
We start with a standard definition of validated agreement~\cite{VABA,
CC}.
Then, as an intermediate state, we define an \emph{Optimisitc}
validated agreement that gives up strong termination in order to
achieve halting and better message complexity in the best case (i.e.,
synchronous periods).
Finally, we define the \emph{distributed ledger} problem, which is a
generalization of the optimistic agreement into a multi-shot problem.

\paragraph{Validated asynchronous agreement.}
% Every Blockchain and SMR system is constructed, in one way or another,
% from multiple instances of a single-shot Agreement protocol.
% The main property of such protocol is the guarantee that no two party
% decide on a contradicting value:
A \emph{validated asynchronous agreement} is single-shot problem in
which honest parties propose values that satisfy a verifiable external validity
condition and agree on a unique such value.
The formal properties are given below:  

\begin{itemize}
    
  \item Agreement: All honest parties that decide, decide on the
  same value.

  \item Termination: If all correct parties propose externally
  valid values, then all honest parties eventually decide.
  
  \item Validity: If an honest party decides an a value $v$, then $v$
  is externally valid.

\end{itemize}

\noindent Note that the agreement and termination properties are not
enough by themselves to guarantee goodput.
Without external validity, the strongest notion of validity would be \emph{Weak
Validity}~\cite{cachin?mustanfoui?}, allowing
parties to agree on some pre-defined value (i.e., $\bot$)~\cite{}, which is basically 
agreement not to agree.
Moreover, as long as a value satisfies the system's external validity
condition (e.g., no contradicting transactions in a blockchain
system), we do not care if the value was proposed by a byzantine
party.

\paragraph{Optimistically efficient validated asynchronous agreement}

Practical BFT protocols usually optimize for common settings in which the
network exhibits synchrony. Indeed, several
advances in BFT solutions (e.g., RO~\cite{constantinopole},
SBFT~\cite{SBFT}, HotStuff~\cite{hotStuff}) achieve linear communication
complexity -- the optimal -- when the network is synchronous. 
We would therefore like our framework to not impose higher communicatoin
complexity than linear during periods of synchrony.

To this end, we define \emph{optimistic Validated Agreement} that
achives linear complexity during synchronous periods.
Instantiating our framework with the above solutions, we may thus obtain
linear communication cost in the best
case, while paying no more than quadratic cost when faced with asynchrony. 

From a theoretical point of view, we usually measure
message/communication complexity by the total number of messages/bits
sent by honest parties before they all decide.
However, from a system point of view, we are also interested in the
messages sent after a decision is made since it impacts the overall
system performance. 
Therefore, we define communication complexity as follows:


\begin{definition}[Communication complexity]

The communication complexity of an Agreement protocol is the total
number of bits sent by honest parties.

\end{definition}



\noindent In order for the above difinition to make sense, we define
the notion of halting and require all honest parties to eventually
halt.
We say that a party \emph{halts} in an execution of a protocol if
there is a time after which it does not send any messages.
%
% honest A desired property for Agreement protocols that are used in
% side real systems is the ability to halt, i.e., stop sending messages
% after decision is made.
%
Note that the standard way to achieve halting requires 
quadratic communication due to state transfer:
Before halting, a party reliably broadcasts the decision value (with
the required proof) to all parties.
We conjuncture that this quadratic communication is inherent and
cannot be avoided if one wishes to satisfy the standard Agreement,
Termination, and Validity properties defined above.
However, we notice that the above termination property might be too
strong for many systems. 
Usually, all we want is to make sure that any client will be able to
get the decision value and no two clients will ever see
different decision values.
To this end, we refine the termination definition and define
\emph{noticeable termination}. On the one hand, noticeable termination is weak enough to
allow us to avoid the quadratic communication cost induced by the
state transfer in best case scenarios. On the other hand, it is strong
enough to capture the requirements of distributed ledger systems.


The best environment one can hope for is a synchronous
network with no failures.
However, such definition of base case scenarios is not very useful
for fault-tolerant systems.
Intuitively, we want to define a best case scenario that will later
allow us to define and implement optimistic distributed ledgers in
which we want to bound the extra communication complexity byzantine
parties to cause during synchronous periods.
To this end, we assume a pre-defined party $p*$ known to all and say
that a best case scenario is one in which the network is synchronous
and $p*$ is honest.
The formal definition of optimistic efficient asynchronous validated
agreement is below:

\begin{definition}[Optimistic efficient asynchronous validated
agreement]

A protocol for \emph{optimistic efficient asynchronous validated
agreement} must satisfy, in addition to the Agreement and validity
properties defined above, the following properties except with
negligible probability:

\begin{itemize}
  
  \item Halting: Eventually there is a point after which no messages
  are sent by honest parties.
  
  \item Noticeable termination: At least $f+1$ honest parties
  eventually decide.
  
  \item Efficiency: The communication complexity is bounded by
  $O(n^2)$.
  
  \item Optimism: For a designated party $p*$ (known to all), if the network is synchronous and $p*$ is honest,
  then the communication cost is $O(n)$.
  
\end{itemize}

\end{definition}


 

\paragraph{Distributed ledger.}

\DM{I am a bit torn about whether we should position this paper as byzantine
state-machine-replication work or a blockchain work. Perhaps as a middle ground
we can call the SMR problem "the ledger replication" problem?}

The distributed ledger problem is a generalization of the single-shot
agreement into a multi-shot distributed task.
In the \emph{distributed ledger} task, every honest party is input with
a (possible infinite) sequence of externally valid values, and
outputs a sequence of tuples of the form $\lr{sq,v}$, where $sq \in
\{1,…,N\}$ for an arbitrary large $N$ and $v$ is a value.
Note that each output event contains exactly one such tuple.
For any point $t$ in an exaction of a distributed ledger, we denote by
$S(t)$ the highest sequence number $sq$ such that some honest party
outputs $\lr{sq,v}$ for some $v$ before time $t$. 
\DM{I think there might be a minor problem with this definition. In particular,
say that before GST, a leader issues one google proposals, all of which become
committed but only the leader knows that. Wouldn't it take one google (times
$n$) messages after GST for all honest parties to output these google decisions?}
In the rest of the paper we sometimes refer to the sequence number
$sq$ as a \emph{slot} number.
%
An implementation of a \emph{distributed ledger} must satisfies the
following properties:

\begin{itemize}
  
  \item Integrity: For every $sq \in \{1,…,N\}$, an honest party
  outputs at most one tuple $\lr{sq,v}$.
  
  \item Noticeable termination: For every $sq \in \{1,…,N\}$, at least
  $f+1$ honest parties eventually output a tuple $\lr{sq,v}$ for some $v$.
  
  \item Agreement: For every $sq \in \{1,…,N\}$, if two honest parties
  output $\lr{sq,v}$ and $\lr{sq,v'}$, then $v = v’$.
  
  \item Halting: Eventually there is a point after which no messages
  are sent by honest parties.
  
\end{itemize}


\paragraph{Optimistically efficient asynchronous distributed ledger.} 
 

As mentioned before, we are interested in optimistic solutions that,
on the one hand, guarantee progress during asynchronous network
periods and adaptive DoS attacks, and on the other hand, leverage
synchronous network periods to achieve good performance.
The standard way to capture these desired properties is by assuming a
\emph{global stabilization time (GST)}, which is defined for
partially synchronous communication models.
% The performance of our framework inherently depends on the specific
% protocol it is instantiated with.
Roughly speaking, our framework guarantees that after GST the
communication complexity of every decision is as good as the communication
complexity of the the specific protocol it is instantiated with.
Before GST (when the instantiated protocol does not guarantee
progress) our framework increases it by no more than a factor $n$.

Specifically, when our framework is instantiated with protocols whose common
mode has linear communication complexity like SBFT or HotStuff, our framework aims to
achieve quadratic communication complexity before GST and linear
after GST.
Unfortunately, failures may happen after GST as well, so we
need to be able to account for the extra cost they cause. 
To this end, we define an optimistic
efficient asynchronous distributed ledger as follows:

\begin{definition}[optimistic efficient asynchronous distributed
ledger]

In addition to the Integrity, Noticeable termination, Agreement, and
Halting defined above, a protocol for \emph{optimistic efficient
asynchronous distributed ledger} must satisfy the following
properties except with negligible probability:

\begin{itemize}
  
  \item Efficiency: For every time $t$, the number of messages sent by
  honest parties is bounded $O(S(t)n^2)$.
  
  \item Optimism: For every time $t$ after GST, the number of
  messages sent by honest parties after GST and before $t$ is
  $O( (S(t) - S(GST))n + f(n^2)  )$.
 

  
\end{itemize}
% 
% Optimism: If the execution is synchronous, than for every time t, the number of messages sent by honest parties is O( S(t)n + fn^2 ).
% More precisely,   O( ( max(1, S(t))n + min(S(t)+1,f)n^2  ).
%  
% Alternative Optimism: For every time t after GST, the number of messages sent among honest parties between t and GST is O( (S(t) – S(GST))n + fn^2  ).
\end{definition}  




Note that when the number of slots after GST ($S(t) -
S(GST)$) is much bigger than $f$, the quadratic extra cost induced by
faulty parties ($f(n^2)$) is negligible and we get (almost) linear
communication cost per slot after GST.
A lower bound in~\cite{VABA, Ittai et al.} shows that $O(n^2)$ is the
best communication complexity one can hope for in asynchronous
networks, and clearly it is impossible to achieve termination with
less than $O(n)$ messages (in order to decide you need to hear at
least one message).
Therefore, to the best of our knowledge, our framework, yields the
first optimal optimistic distributed ledger protocol for both benign
and byzantine failures.

\sasha{Note that here we must separate the execution from the
replication.}\ittai{good point - we will need to elaborate on this}







==> ProblemDefinitionBeforePLDI.tex <==
% \subsection{Single-shot Agreement}
% 
% We use the VABA version because this what we need for a distributed
% ledger.
% 
% Maybe merge 3.2 and 3.3 in order to give some intuition for VABA
% definition.

% Halting.

\subsection{Problem Definitions}
We start with a standard definition of validated agreement~\cite{VABA,
CC}.

\begin{definition}[Validated Agreement]
Each party has some externally validated input.

\begin{itemize}

    
  \item Agreement: All honest parties that decide, decide on the
  same value.

  \item Decision: all honest parties eventually decide.
  
  \item Termination: all honest parties eventually terminate.
  \sasha{confusing - termination usually means what tou defined by
  decision. I prefer Halting.} \sasha{Moreover, standard definitions
  do not have Halting.}
  
  \item Validity: If an honest party decides an a value $v$, then $v$
  is externally valid.
  
  

\end{itemize}
\end{definition}

We now define a new variant of validated agreement that has weaker decision and termination properties.
In order to avoid quadratic costs, we do not explicitly reach a \emph{Terminating state} (where all honest terminate). Instead, we reach a state where no new message is sent or received by any honest party. We call this a \emph{Quiescent State}.


\begin{definition}[Quiescent Validated Agreement]
Each party has some externally validated input.

\begin{itemize}

    
  \item Agreement: All honest parties that decide, decide on the
  same value.

  \item Noticeable decision: at least $f+1$ correct parties eventually decide.
  
  \item Weak Termination: all honest parties eventually reach a
  quiescence state.\sasha{need to define quiescence state.}
  
  \item Validity: If an honest party decides an a value $v$, then $v$
  is externally valid.
  
 
\end{itemize}
\end{definition}

\noindent Finally, we define a new variant of validated agreement that is also optimistically efficient given synchrony and an honest leader $p*$.

\begin{definition}[Quiescent Validated Agreement with  optimistic efficiency given a leader $p*$]
Each party has some externally validated input.

\begin{itemize}

    
  \item Agreement: All honest parties that decide, decide on the
  same value.

  \item Noticeable decision: at least $f+1$ correct parties eventually decide.
  
  \item Weak Termination: all honest parties eventually reach a quiescence state.
  
  \item Validity: If an honest party decides an a value $v$, then $v$
  is externally valid.
  
  \item Efficiency: The communication complexity is bounded by
  $O(n^2)$.
  
  \item Optimism given $p*$ and synchrony: If the network is synchronous and $p*$ is honest,
  then the communication cost is $O(n)$.
 
\end{itemize}
\end{definition}

\newpage
Then, as an intermediate state, we define an \emph{Optimisitc}
validated agreement that gives up strong termination in order to
achieve halting and better message complexity in the best case (i.e.,
synchronous periods).
Finally, we define the \emph{distributed Ledger} problem, which is a
generalization of the optimistic agreement into a multi-shot problem.

\paragraph{Validated asynchronous agreement.}
% Every Blockchain and SMR system is constructed, in one way or another,
% from multiple instances of a single-shot Agreement protocol.
% The main property of such protocol is the guarantee that no two party
% decide on a contradicting value:
A \emph{validated asynchronous agreement} is single-shot problem in
which honest parties propose externally valid values and agree on a unique such
value.
The formal properties are given below:  

\begin{itemize}
    
  \item Agreement: All honest parties that decide, decide on the
  same value.

  \item Termination: If all correct parties propose externally
  valid values, then all honest parties eventually decide.
  
  \item Validity: If an honest party decides an a value $v$, then $v$
  is externally valid.

\end{itemize}






\noindent Note that the agreement and termination properties are not
enough by them self to guarantee real progress of any Blockchain system that
built on top of the Agreement abstraction.
Without external validity, parties are allowed to agree on some
pre-defined value (i.e., $\bot$)~\cite{}, which is basically an
agreement not to agree.
Moreover, as long as a value satisfies the system's external validity
condition (e.g., no contradicting transactions in a blockchain
system), we do not care if the value was proposed by a byzantine
party.

\paragraph{Optimistic efficient validated asynchronous agreement}

Although tolerating asynchronous periods is an important property for
online systems operating on top of the Internet, real systems
usually choose to give up this capability due to the higher
communication complexity it causes. 
To this end, we define \emph{optimistic Validated Agreement} that
exploit synchronous periods for better complexity.
Moreover, by instantiating our framework with the state of the art 
linear partially synchronous protocol form~\cite{VABA, hotStuff}, we
wish to achieve the optimal linear communication cost in the best
case, while paying no more than quadratic cost in the worst case.


From a theoretical point of view, we usually measure
message/communication complexity by the total number of messages/bits
sent by honest parties before they all decide.
However, from a system point of view, we are also interested in the
messages sent after a decision is made since it impacts the overall
system performance. 
Therefore, we define communication complexity as follows:


\begin{definition}[Communication complexity]

The communication complexity of an Agreement protocol is the total
number of bits sent by honest parties.

\end{definition}



\noindent In order for the above difinition to make sense, we define
the notion of halting and require all honest parties to eventually
halt.
We say that a party \emph{halts} in an execution of a protocol if
there is a time after which it does not send any messages.
%
% honest A desired property for Agreement protocols that are used in
% side real systems is the ability to halt, i.e., stop sending messages
% after decision is made.
%
Note that the standard way to achieve halting requires inherent
quadratic communication due to the so called state transfer.
Before halting, a party reliably broadcasts the decision value (with
the required proof) to all parties.
We conjuncture that this quadratic communication is inherent and
cannot be avoided if one wishes to satisfy the standard Agreement,
Termination, and Validity properties defined above.
However, we notice that the above termination property might be too
strong for many systems. 
Usually, all we want is to make sure that any client will be able to
get the decision value and no two clients will ever see
different decision values.
To this end, we refine the termination definition and define
\emph{noticeable termination} that on the one hand weak enough to
allow as to avoid the quadratic communication cost induced by the
state transfer in best case scenarios, and on the other hand strong
enough to catch the requirements of Blockchain systems.


The best environment one can hope for is a synchronous
network with no failures.
However, such definition of base case scenarios is not very useful
for fault-tolerant systems.
Intuitively, we want to define a best case scenario that will later
allow us to define and implement optimistic distributed ledgers in
which we want to bound the extra communication complexity byzantine
parties are able to cause during synchronous periods.
To this end, we assume a pre-defined party $p*$ known to all and say
that a best case scenario is one in which the network is synchronous
and $p*$ is honest.
The formal definition of optimistic efficient asynchronous validated
agreement is below:

\begin{definition}[Optimistic efficient asynchronous validated
agreement]

A protocol for \emph{optimistic efficient asynchronous validated
agreement} must satisfy, in addition to the Agreement and validity
properties defined above, the following properties except with
negligible probability:

\begin{itemize}
  
  \item Halting: Eventually there is a point after which no messages
  are sent by honest parties.
  
  \item Noticeable termination: At least $f+1$ honest parties
  eventually decide.
  
  \item Efficiency: The communication complexity is bounded by
  $O(n^2)$.
  
  \item Optimism: If the network is synchronous and $p*$ is honest,
  then the communication cost is $O(n)$.
  
\end{itemize}

\end{definition}


 

\paragraph{Distributed ledger.}

The distributed ledger problem is a generalization of the single-shot
agreement into a multi-shot distributed task.
In the \emph{distributed ledger} task, every honest party inputs with
a (possible infinite) sequence of externally valid values, and
outputs a sequence of tuples of the form $\lr{sq,v}$, where $sq \in
\{1,…,N\}$ for an arbitrary large $N$ and $v$ is a value.
Note that each output event contains exactly one such tuple.
For any point $t$ in an exaction of a distributed ledger, we denote by
$S(t)$ be the highest sequence number $sq$ such that some honest party
outputs $\lr{sq,v}$ for some $v$ before time $t$. 
In the rest of the paper we sometimes refer to the sequence number
$sq$ as a \emph{slot} number.
%
An implementation of a \emph{distributed ledger} must satisfies the
following properties:

\begin{itemize}
  
  \item Integrity: For every $sq \in \{1,…,N\}$, an honest party
  outputs at most one tuple $\lr{sq,v}$.
  
  \item Noticeable termination: For every $sq \in \{1,…,N\}$, at least
  $f+1$ honest parties eventually output a tuple $\lr{sq,v}$ for some $v$.
  
  \item Agreement: For every $sq \in \{1,…,N\}$, if two honest parties
  output $\lr{sq,v}$ and $\lr{sq,v'}$, then $v = v’$.
  
  \item Halting: Eventually there is a point after which no messages
  are sent by honest parties.
  
\end{itemize}


\paragraph{Optimistic efficient asynchronous distributed ledger.} 
 

As mentioned before, we are interested in optimistic solutions that
on the one hand guarantee progress during asynchronous network
periods and adaptive DoS attacks, and on the other hand exploit
synchronous network periods to achieve great performance.
The standard way to capture these desired properties is by assuming a
\emph{global stabilization time (GST)}, which is defined for
partially synchronous communication models.
% The performance of our framework inherently depends on the specific
% protocol it is instantiated with.
Roughly speaking, our framework guarantees that after GST the
communication complexity of every decision is as good as the communication
complexity of the the specific protocol it is instantiated with, and
before GST (when the instantiated protocol does not guarantee
progress) our framework increases it by no more than a factor of $n$.

Therefore, when instantiated with a protocol with a linear
communication complexity~\cite{VABA, hotstuff}, our framework aims to
achieves quadratic communication complexity before GST and linear
after GST.
Unfortunately, failures may happen after GST as well, so we
need to be able to bound the extra cost they can force on the system.
To this end, we define an optimistic
efficient asynchronous distributed ledger as follows:

\begin{definition}[optimistic efficient asynchronous distributed
ledger]

In adaption to the Integrity, Noticeable termination, Agreement, and
Halting defined above, a protocol for \emph{optimistic efficient
asynchronous distributed ledger} must satisfy the following
properties except with negligible probability:

\begin{itemize}
  
  \item Efficiency: For every time $t$, the number of messages sent by
  honest parties is bounded $O(S(t)n^2)$.
  
  \item Optimism: For every time $t$ after GST, the number of
  messages sent by honest parties after GST and before $t$ is
  $O( (S(t) - S(GST))n + fn^2  )$.
 

  
\end{itemize}
% 
% Optimism: If the execution is synchronous, than for every time t, the number of messages sent by honest parties is O( S(t)n + fn^2 ).
% More precisely,   O( ( max(1, S(t))n + min(S(t)+1,f)n^2  ).
%  
% Alternative Optimism: For every time t after GST, the number of messages sent among honest parties between t and GST is O( (S(t) – S(GST))n + fn^2  ).
\end{definition}  




Note that when the number of slots started after GST($S(t) -
S(GST)$) is much bigger than $f$, the quadratic extra cost induced by
faulty parties ($fn^2$) is negligible and we get (almost) linear
communication cost per slot after GST.
A lower bound in~\cite{VABA, Ittai et al.} shows that $O(n^2)$ is the
best communication complexity one can hope for in asynchronous
networks, and clearly it is impossible to achieve termination with
less than $O(n)$ messages (in order to decide you need to hear at
least one message).
Therefore, to the best of our knowledge, our framework, yields the
first optimal optimistic distributed ledger protocol for both, benign
and byzantine failures.

\sasha{Note that here we must separate the execution from the
replication.}\ittai{good point - we will need to elaborate on this}







==> algReconsutrction.tex <==
\section{Partially Synchronous Algorithm Reconstruction (Section 5)}
\label{sec:originalAlg}

For completeness, we show how to use the LBV
abstraction to reconstruct a variant of the partially
synchronous base Agreement algorithm that the LBV abstraction was
instantiated with.
To this end, we assume the base algorithm provides two methods:
\emph{getLeader} and \emph{getTimeout}.
These methods should implement the logic used by the base algorithm
to map designated leaders to views and set their timeouts,
respectively. 
In particular, \emph{getLeader(v)} gets a view $v$ and returns a
party $p_i \in \{ p_1\dots,p_n\}$, and \emph{getTimeout(v, S)} gets a view
$v$ together with a state $S$ and returns a timeout. 
% The timeout should partially be large enough such that after GST a
% \propose invocation returns within the timeout.

The pseudocode appears in Algorithm~\ref{alg:reconSS}.
% Using these methods and the LBV abstraction, we present the
% pseudocode of the reconstruction in Algorithm~\ref{alg:reconSS}.
The protocol proceeds in views.
Timeouts are used in order to demote a leader who was unable to drive
progress.
At the beginning of every view, parties first get the leader and the
timeout of the current view, and then invoke \propose in the leaders
LBV instance and a timer to monitor the leaders progress.
If the \propose invocation returns $v$ before the timer expires, then
$v$ is decided.
In any case, whether the \propose invocation returns or
the timer expires, a \vc is invoked in order to update the state and
safely proceed to the next view.

Note that the algorithm forms a properly composed execution of the LBV
instances, and thus Validity and Agreement are trivially satisfied by
the Safety properties required by the LBV abstraction.
As any protocol in the partially synchronous model, the termination
of the algorithm requires a long enough synchronous period in which all
correct parties execute the same view. 

\begin{figure}[th]
    \begin{center}
        \includegraphics[width=0.48\textwidth]{reconstruction.png}
    \end{center}
    \caption{An illustration of the reconstruction of the partially synchronous
    algorithm. The LBV and timer are invoked in parallel at the same time; when either
    the LBV \propose returns or the timer expires, then the parties move on to the next view,
    possibly deciding.}
    \label{fig:ASprotocol}
\end{figure}  





\input{SSOrigAgreement.tex}


\section{Leader-Election Implementation (Section 6.1)}
The leader election is similar to that of \cite{vaba} and
\cite{Cachin2000RandomOI}.
When a party invokes \emph{elect}, it signs the instance's
identification and broadcasts its share.
When a correct party collects $f+1$ valid shares, it combines them
to a threshold signature, hashes the signature to get a pseudo
random value, and returns the value modulo $n$ to get a random leader.

As the threshold signature is generated from $f+1$ valid shares, all
correct parties eventually generate it provided that at least $f+1$
correct parties invoke \emph{elect}, satisfying \emph{L-Termination}.
Due to the nature of threshold cryptography, the generated
threshold signature is the same for all correct
parties~\cite{boneh2001short}, and since the hash and modulo functions
are deterministic, all parties agree on the electing leader,
satisfying \emph{L-Agreement}.
For formal analysis of \emph{L-Validity} and \emph{L-Unpredictability}
please refer to~\cite{Cachin2000RandomOI, cachin2001secure, vaba}.




==> framework_2.tex <==
\section{Framework For Single-Shot Agreement}
\label{sec:framework}


\DM{Adding some thoughts for discussion:}
\newcommand{\grade}[1]{$grade(#1)$}
Our framework for asynchronous agreement is based on repeatedly variating over a
classical primitive called \emph{graded-cast}. 
Graded-cast operates, grade-by-grade, using a framework due to Bracha~\cite{??}: 
In grade $(g+1)$, when a party collects identical \grade{$g$} outputs from a
quorum ($2f+1$) of parties, it delivers a \grade{$g+1$} output carrying the value.
In a leaderless mode, parties broadcast their outputs to each other, and when
a party collects $f+1$ identical \grade{$g$} outputs, it echoes the value via a broadcast to all.
In a leader-based variant, a leader serves as `hub' and collects/distributes
inputs from/to a quorums of parties. 
%
The two key properties of ``grading'' when $g > 1$ are:
(i) if any two honest parties deliver \grade{$g$} output $v$ and $v'$
respectively, then $v=v'$.
(ii) if an honest party delivers a \grade{$g$} output $v$, then at least $f+1$ honest
parties deliver grade-$(g-1)$ output $v$. 

A variant of graded-cast that uses cryptographic signatures and outputs a
\emph{provable} graded-output, where the output includes an aggregate of
$2f+1$ signed messages from the previous grade.

Graded-cast is guaranteed to terminate if $2f+1$ honest parties participate.
Additionally, in instances where such API is allowed, Termination is conditioned
on no honest party invoking `abandon()'.

The first rounds of graded-cast variants differ in the validity condition they
impose on accepting values as follows: 

\begin{description}

	\item[ Validity-1]: 
	Accept an identical value from $f+1$ (similar to higher grades)

	\item[ Validity-2]: 
	Accept an externally-valid value from a designated primary

	\item[ Validity-3]: 
	Accept an identical value from $f+1$ (similar to higher grades) or
	an externally-valid value

\end{description}

We can succinctly introduce all of our primitives (except leader election, see
below) as instances of grade-cast with the above validity conditions. The
framework primitives are as follows:

	\begin{description} 
	\item[Barrier]: The first round uses Validity-1 on $\bot$ (i.e., simply signal
arrival). Use 2 grades. 
	\item[View-Change]: The first round uses Validity-1 on externally-valid input. Use only 1 grade.
	\item[Primary-Backup]: The first round uses Validity-2 on externally-valid input. Use 3 grades (?).
	\item[Trigger]: The first round uses Validity-3 on $\bot$ (arrival) or a
provable trigger-sync. Use 2 grades.
	\end{description} 


\DM{to here.}



primitives:
\emph{Leader based protocol (LBP)}, \emph{view-change},
\emph{leader-election}, \emph{barrier}, and
\emph{view-change-trigger}.
In this section, we define a simplified version of their properties
that is sufficient for implementing single-shot asynchronous
Agreements: the standard and the optimistic efficient versions.
Later, in Section~\ref{}, we extend their required properties in order
to implement distributed ledgers.
We start, in Section~\ref{sub:decoupling}, with the \emph{Leader based
protocol (LBP)} and \emph{view-change} primitives, which are implicitly
implemented in every practical protocol in the partially synchronous
model we are aware of.
Then, in Section~\ref{sub:auxiliary}, we define the three additional
primitives we use in our algorithms.

\DM{not sure this is the right place for the following paragraph:}
As mentioned above, the specific implementation details of the
primitives as well as the specific model assumption made for their
correction are abstracted away by the primitives' specification.
The correction of our algorithms does not require any additional
assumptions.
Therefore, the results in this paper are very generic and apply for
many models.
In particular, if the primitives' implementation assumes $n=3f+1$
parties, computationally bounded adversary, and byzantine failures,
then all our results apply to this model.
And if the primitives' implementation assumes $n=2f+1$ parties and
crash failures then our algorithm are correct for this model.  



\subsection{Decoupling partially synchronous agreement protocols}
\label{sub:decoupling}
\arik{
  This is no longer decoupling, but rather unrolling. The parties complain,
  invoke a VC and then run another LBP.
}
To the best of our knowledge, all practical protocols in the
partially synchronous model use the following approach: a
designated leader is trying to convince a sufficient quorum of the
parties to adopt and then commit its proposal.
\DM{I believe that the (new) introduction positions this better : we provide a boosting
framework for (abandonable) single-shot primary-backup consensus solutions. No?}
If the leader menages to do it fast enough then its proposal is
decided. 
Otherwise, the parties complain and safely replace the leader to the
next one in line (usually there is some pre-defined order of the
leaders).
In order to be able to turn a partially synchronous solution into an
asynchronous one we decouple the leaders' protocol to drive a decision
from the leader replacing protocol into two primitives: \emph{\LBP}
and \emph{view-change}.
\arik{
  into a \emph{leader-view-based-protocol (LVBP)} primitive.
}

As defined below the properties of the \emph{\LBP} and
\emph{view-change} primitives are defined over \emph{alternate
executions} in which parties alternately invoke them, where the
output form one is the input for the other.
%
%
% \ldots\ldots\ldots 
% 
% properties are defined over executions
% in which parties alternately invoke the \emph{\LBP} and the
% \emph{view-change} abstractions, where the output form one is the
% input for the other.
% In Section~\ref{subsec:liveness}, we show how this abstraction can be
% used, together with few other simple primitives, to construct two
% general protocols for agreement; one for the asynchronous and one for
% partially synchronous communication models.
% In Section~\ref{subsec:practical}, we propose a practical
% constructions that combine these protocols in order to achieve good
% throughput during synchronous periods (best case), while
% guarantying progress during asynchronous periods (worse case).
% 
% 
% \subsection{Abstractions}
% \label{subsec:abs}
% 
% In this section we present the abstraction we use for the single shot
% Agreement framework, and in Section~\ref{subsec:practical} we slightly
% strengthen these abstractions for the state machine replication
% (SMR) framework.
Every instance of the primitives is parametrized with an
identification $id$, which contains information used by the
high-level agreement protocol built on top of them, and the \LBP\ is
also parametrized with a leader name.
An illustration of the primitives' API appears in
Figure~\ref{fig:abs}.
The leader of an \LBP\ invokes a \emph{propose} operation where all
other parties invoke an \emph{approve} operation and might 
additionally invoke \emph{abandon}.
Both \emph{propose} and \emph{approve} operation gets a \emph{state}
parameter as an input, and return a tuple consists of a \emph{state}
and a value $v \in  \mathcal{V} \cup \{\bot\}$ \arik{they now only return state}.
In an instance of a \emph{view-change} primitive, all parties invoke
\emph{VC} operation with the \emph{state} and the value that were
returned from the previous \LBP, and receive as a return value a new
tuple of \emph{state} and value. \arik{Once an approve returns, a VC is
invoked, such that the state input to the VC is the output of the previous
approve.}
The \emph{state} parameter that is passed to and returned from both
primitives, by all parties, consists of all the necessary
information required by the specific implementation (e.g., a safe
value for a leader to propose or a function all parties use to check
if the proposed value is safe).
The \emph{value} parameter is either a value in the domain
$\mathcal{V}$ or $\bot$, which intuitively signals a \emph{commit}
event.

% consists of 4 fields:
% \begin{itemize}
%   
%   
%   \item A \emph{value} and a \emph{proof} for every leader to propose
%   in the \LBP\ abstraction.
%   
%   \item A function \emph{VC-checker}, that is maintained by the
%   \emph{view-change} abstraction, and used by parties in the \LBP\ to
%   check if the value and proof are valid. 
%   It gets a view number, a value, and a proof, and returns \emph{true}
%   or \emph{false}.
%   
%   \item A function \emph{LBP-checker} that is used by the view-change
%   abstraction to check that each party's input is a valid output from
%   the \LBP. 
%   It gets a value, a status, and a proof, and returns \emph{true}
%   or \emph{false}.
%   
% \end{itemize}
%
%\begin{figure}[th]
%    \centering
%    \begin{subfigure}[t]{0.49\textwidth}
%        \centering
%        \includegraphics[width=3.2in]{LBP.png}
%        \caption{}
%         \label{}
%    \end{subfigure}%
%    ~
%    \begin{subfigure}[t]{0.49\textwidth}
%        \centering
%        \includegraphics[width=2in]{VC.png}
%        \caption{}
%        \label{}
%    \end{subfigure}
%    \caption{}
%    \label{fig:abs}
%\end{figure}

\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{LVBP.png}
  \end{center}
  \caption{API for the \emph{LVBP} primitive.}
  \label{fig:abs}
\end{wrapfigure}

\paragraph{Alternate executions of the primitives.}
\arik{
  Since the different instances of the \emph{LVBP} need to communicate
  with each other, the properties the primitive must satisfy is
  defined only over \emph{alternate executions} in which honest parties
  alternate their participation in the primitives s.t. the output
  of one instance is the input of the other. Figure~\ref{fig:ESprotocol}
  illustrates such execution. The \emph{state} is defined by
  the specific implementation, and the initial \emph{state} is given
  as input to the system, and then passed from the output
  of one \emph{LVBP} to the next.
}
Since the implementations of the \LBP\ and view-change
primitives requires them to communicate with each other (e.g., a
party cannot know if the leaders value is safe without getting
information from the previous view-change), we do not define the
properties of each of the primitives as stand alone abstractions.
Instead, the properties these primitives must satisfy are defined
only over \emph{alternate executions} in which honest parties
alternate their participation in a \LBP\ and \emph{view-change}
primitives s.t.\ the output from one is the input for the other.
% Such execution starts with a \LBP\ with $view = 1$ and an arbitrary
% leader, and followed by a \emph{view-change} with $view = 1$.
% Then, it continuous with a \LBP\ with $view = 2$ (and an arbitrary
% leader), followed by a \emph{view-change} with $view = 2$, and so on.
Figure~\ref{fig:ESprotocol} illustrates such execution.
The first primitive in an alternate executions is always a \LBP\ and
the initial \emph{state} parameter passed to its \emph{approve(state)}
and \emph{propose(state)} operations is defined by the specific
implementation.
For all other instances of the \LBP\,
\emph{approve(state)} and \emph{propose(state)} operations get the
state that was returned by the $VC$ operation of the previous
\emph{view-change} instance.
In all instances of the \emph{view-change} abstraction, the $VC$
operation gets a $state$ and a $value$ that were returned by the
\emph{approve} operation in the previous \LBP\ instance.

\begin{figure}[th]
    \centering
        \includegraphics[width=5in]{alternateExec2.png}
        \caption{}
    \label{fig:ESprotocol}
\end{figure}

% 
% In this section we show that an execution in which parties
% alternatively invoke \LBP\ and \emph{view-change} s.t.\ the output
% from one is the input for the other satisfies the agreement and
% validity properties regardless of who is the leader of every \LBP\
% instance.
% Such execution starts with a \LBP\ with $view = 1$ and an arbitrary
% leader, and followed by a \emph{view-change} with $view = 1$.
% Then, it continuous with a \LBP\ with $view = 2$ (and an arbitrary
% leader), followed by a \emph{view-change} with $view = 2$, and so on.
% 
% For every instance of the \LBP, the
% \emph{invoke} operation by each party $p_i$ gets a state $state_i$,
% and the leader $p_l$ proposes $state_l.value$ and $state_l.proof$.
% For every view $view > 1$ and party $p_i$, $state_i$ is the state
% returned by the \emph{view-change} with view $view - 1$.
% As for view $view = 1$, for every party $p_i$, $state_i.value = v_i$
% and $state_i.\emph{VC-checker}(0,v,\sigma) = \emph{true}$ if and only
% if $v$ is externally valid.
% For every party $p_i$, the \emph{invoke} operation of the view-change
% abstraction with a view $view \geq 1$ gets a state $state_i$,
% $value_i$, $status_i$, and $proof_i$ that was returned by the
% \LBP with view $view$.


\paragraph{Properties.}

Properties that must be satisfied by the \emph{leader-view-based-protocol}
primitive:
\begin{itemize}
  \item \textbf{\emph{approve}-Termination:} If the leader of the instance is
  honest, all honest parties invoke \emph{approve}, and no honest
  party invokes \emph{abandon}, then the leader's \emph{propose} invocation
  eventually returns.
   
  \item \textbf{\emph{VC}-Termination:} If all honest parties invoke \emph{VC},
  then all \emph{VC} invocations by honest parties eventually return.

  \item \textbf{Completeness:} If a \emph{propose} invocation by an
  honest leader returns, then all honest parties' \emph{VC}
  invocations return \arik{some?} \emph{value} $v \neq \bot$.

  \item \textbf{Validity:} If a \emph{VC} invocation
  by an honest party returns a value $v \neq \bot$,
  then $v$ is externally valid.
  
  \item \textbf{Agreement:} If the invocation of \emph{VC} of party $p_i$
  in instance $k$ returned value $v \ne \bot$, and the invocation of \emph{VC} of party $p_j$
  in instance $l$ returned value $v' \ne \bot$, then $v = v'$.

\end{itemize}

\paragraph{Safety of alternate executions.} Note that by the required
validity and agreement properties, any Agreement protocol that is
built on top of an alternate execution of the primitives can
safely decide on the value returned from any of the instances in
the execution.
In the next section we show how to guarantee \emph{liveness} for
Agreement on top of legal executions.

\ittai{that was too fast for me. I think this is more than a "note" - it should be a theorem, mainly the notion of "any Agreement protocol that is built on top of a legal
execution" should be stressed.}
\DM{Me too :-) . ANY agreement protocol?? if it does nothing? ..}

\sasha{I agree. We need to define better alternate executions, and
prove a general safety theorem for a family of algorithm that uses
them.}

\subsection{Auxiliary primitives}
\label{sub:auxiliary}


To give a general construction for the asynchronous networking model
we use three additional primitives, \emph{leader-election},
\emph{barrier}, and \emph{view-change-trigger} ,which are also
parametrized with an identification $id$.
As for the \LBP\ and \emph{view-change} primitives, the implementation
details and assumptions are abstracted away.

\paragraph{Barrier.}
As the name suggest, the barrier abstraction makes sure that honest
parties wait to each other before moving forward.
%  An illustration of its API appears in Figure~\ref{fig:barrier}.
All parties may invoke two operations: \barrierready and
\barriersync.
Below we define the properties each barrier implementation must
satisfy:

\begin{definition}

An implementation of the Barrier primitive must satisfy the
following properties:

\begin{itemize}
  
  \item B-Coordination: No \barriersync invocation by an
  honest party returns before $f+1$ honest parties invoke
  \barrierready.
  
  \item B-Termination: If all honest parties invoke
  \barrierready then all \barriersync invocations by honest
  parties eventually return.
  
  \item B-Agreement: If some \barriersync invocation by
  honest party returns, then all \barriersync invocations by honest
  parties eventually return.
  
\end{itemize}

\end{definition}

\paragraph{Leader election.}
%
The \emph{Leader-election} primitive exposes one operation,
\elect, to elect a unique leader.
The formal properties are given below.

\begin{definition}

An implementation of the Leader-election primitive must satisfy the
following properties:

\begin{itemize}
  
  \item {L-Termination:} If $f+1$ honest parties invoke
  \elect, then all invocations by honest parties eventually return.
  
  \item {L-Agreement:} All invocations of \elect by honest
  parties that return, return the same party.
  
  \item {L-Validity:} If an invocation of \elect by an
  honest party returns, it returns a party $p$ with probability $1 /
  |\Pi|$ for every $p \in \Pi$.
  
  \item {L-Unpredictability:} The probability of the adversary
  to predict the returned value of an \elect invocation by an
  honest party before any honest party invokes \elect is at most $1
  / |\Pi|$.
  
\end{itemize}


\end{definition}


\paragraph{View-change trigger.}

Intuitively, the purpose of the view-change trigger primitive is to
make sure honest parties do not invoke the next \emph{view-change}
primitive if $f+1$ honest parties have decided. 
This is important in order to satisfy the halting property.
All parties may invoke two operations: \emph{trigger()} and
\emph{trigger-sync()}.
The definition is given below:

\begin{definition}

An implementation of the view-change trigger primitive must satisfy
the following properties:

\begin{itemize}
  
  \item T-Coordination: No trigger-sync() invocation by an
  honest party returns before some honest parties invoked
  trigger().
  
  \item T-Termination: If $f+1$ honest parties invoke
  trigger() then all trigger-sync() invocations by honest
  parties eventually return.
  
\end{itemize}

\end{definition}

   

 
\noindent In appendix~\ref{app:} we give some example implementations
of these primitives under different assumptions.



==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

==> introductionBeforePLDI.tex <==
\section{Introduction DRAFT}
\label{sec:intro}


This paper introduces a new framework for the software design of fault tolerant
state machine replication systems. We propose new abstract types that
encapsulate the core of the single shot  Primary-Backup consensus paradigm. Our framework allows to take any implementation of our abstract single-shot Consensus type and make non-trivial use of it in order to transform it into a robust state machine replication system and boost its liveness and performance.
\sasha{Need to talk about abstracting model assumption.}

Our approach provides three significant benefits: a new generic scheme for \emph{SMR boosting}, a new generic \emph{liveness boosting} technique and a new generic \emph{liveness boosting technique with optimistic efficiency}:
\begin{itemize}
    
    \item \textbf{SMR Boosting}. We define a new abstract single shot
    consensus encapsulation.\sasha{Its is even less than this -
    we encapsulate a single round within a single shot
    consensus} Ours abstraction has a
    subtle \emph{noticeable termination} property that is weaker than
    traditional consensus abstractions. \sasha{I think this is not
    the right place to talk about noticeable termination - this is
    only relevant in order to get linear complexity in the best case.
    Currently, you do not talk about optimal linear complexity at
    all\ldots} 
    Nevertheless we provide a generic protocol to transform (boost) any implementation of our single-shot abstraction to a multi-shot State Machine Replication system in an efficent manner that avoids un-necessary quadratic communications. We note that our boosting technique is \emph{adversary agnostic}. For example it applies to both abstractions that are resilient to byzantine corruptions and to those that are resilient to only omission failures.
    
    \item \textbf{Liveness Boosting}. The main power of our abstract consensus encapsulation is that it allows to perform \emph{Liveness Boosting} in an asymptotically optimal manner. Liveness boosting is a generic protocols that takes any implementation of our single-shot abstraction that is \emph{safe} in asynchrony but \emph{live}
only in synchrony and  \textbf{boosts} it to a protocol that is both live and safe
in asynchrony.  Briefly, Liveness Boosting works by
operating $n$ concurrent instances of a consensus abstraction, each
with a different designated leader. Then it carefully waits for a constant
fraction to complete, and selects one instance in retrospect at random, guaranteeing success with constant
probability.
%
We show that the overhead of our boosting technique is asymptotically optimal. Two examples: (1) we show how HotStuff can be boosted to "async hotstuff": a SMR system that is live and safe in asynchrony and for each block has the same word and communication complexity as the best single shot protocol (VABA). (2) we show how Raft can be boosted to "async Raft": the first SMR system that can tolerate $n=2f+1$ omission failures and be both live and safe in asynchrony.
    
    \item \textbf{Liveness Boosting with optimistic efficiency}.
    \sasha{what about Halting?} Our Liveness boosting technique has
    the disadvantage of operating $n$ concurrent instances of the underlying Consensus abstraction. While this provides stronger liveness guarantees, it
also imposes a performance overhead compared to partial synchrony solutions
during periods of synchrony.
%    
    To overcome this gap, we extend the framework with \emph{Liveness Boosting
with optimistic efficiency}. We generically transform any
of our abstract Consensus types to a State Machine Replication protocol that has obtains the best of both worlds:
(1) it is live even in asynchrony;
(2) It incurs essentially no performance overhead when the
system is synchronous compared to the performance of the underlying 
Consensus type.

\end{itemize}

\newpage

\section{Introduction}
\label{sec:intro}

% “The difference between the difficult and the impossible is that the
% impossible takes a little longer time.”, Lady Aberdeen, 1913.
% \sasha{I guess you refer to FLP impossibility and randomize consensus
% ? I feel that it is a bit overselling, after all we are not the first
% to do it. We are not even the first to give an implementation
% for a randomized algorithm. We need to be careful here.}

% \paragraph{Motivation for Agreement}



Intuitively, the Agreement problem is as follows: a set of
$n$ parties, each of which has an input value, are trying to agree on 
a unique output value despite a subset of the players being faulty. 

% \paragraph{Many different model assumptions that yealds too many
% techniques and different lower bounds}
\DM{the next two paragraphs seem to indicate that our focus is on generic fault
models. I would instead emphasize the follows: We introduce a generic
asynchornous framework, that thwarts adversarial schedules 
for partially-synchornous solutions. Our framework integrates arbitrary
solutions in the partial synchrony settings provided they support two (natural)
primitives, a leader-attempt primitive and view-change pritimive. This is where
I was going with the "impossibility" quote above -- the key contribution is to
bypass the impossibility of asynchronous consensus in a generic
manner.}\sasha{sounds good. I think that talking about the generality
is very important but I agree that these two paragraphs are too long or
come too soon}


However, presenting a protocol that solves the Agreement
problem is a way different story. 
In order to give such solution one must first exactly specify
the model and the assumptions under which the protocol is correct.
Unfortunately, the number of possible assumptions is to many to count.
For example, some standard models assume only crash failures~\cite{}
meaning that faulty players honestly follow the protocol until they
crash, whereas others tolerate byzantine failures~\cite{} that
intentionally try to sabotage the protocol.
But even in the byzantine case, some tolerate arbitrary
behavior~\cite{}, whereas others consider only omission deviations
from the protocol~\cite{}.
As for the correct (non-faulty) players, both altruistic and
rational~\cite{} behaviors are possible assumptions.
Another example is the assumption on the network communication. Some
protocol rely on synchrony for both safety and liveness~\cite{}, some
rely on synchrony only for liveness~\cite{}  (such models are called
partially synchronous), whereas others are fully asynchronous~\cite{}.

% \paragraph{Many protocols for each model}
In addition, every set of different assumptions yields different upper
and lower bounds.
For example, in order to solve Agreement that tolerates crash failures
in partially synchronous systems we need the number of players $n$ to
be at least $2f+1$~\cite{}, where $f$ is the maximum number of failures.
For partially synchronous byzantine agreement, we need to assume $n
\geq 3f+1$~\cite{}, but if we allow the use of cryptographic
signatures and assume synchronous communication it is possible
to solve byzantine Agreement for any $f<n$~\cite{}.
As for the upper bounds, many protocols are proposed in the literature
for every combination of model assumptions, each of which uses a
different technique and achieves different communication and latency
costs.
Fortunately, in the paper abstracts away
the specific model assumptions and implementation details all
together.


% \paragraph{The practical approach is to assume eventoul synchrony}
A landmark result in the theory of reliability is the FLP impossibility
proof~\cite{FLP} of solving Consensus in asynchronous settings. 
Unfortunately, in practical systems, synchronous solutions have the
drawback that a disconnection in the network (even termporary) might compromise
safety.
One approach for circumventing FLP pioneered by Rabin~\cite{Rabin83} and
Ben-Or~\cite{benor83} employs randomization. Employing randomization in protocol
steps allow to increase the probability of termination with each step of the
protocol and to approach one within some known expected bound.
Randomized asynchronous solutions incur quadratic
communication (a recently described tight solution appears in~\cite{VABA}).

Many practical consensus algorithms (for byzantine and crash failures) optimize
for the case of a stable leader with timely communication (with a quorum). In
such ``common mode'', solutions like FaB, Zyzzyva, SBFT, HotStuff, (Byzcoin?) reach
consensus deterministically with linear communication and a small number of
protocol rounds.
More specifically, these protocols are designed for \emph{partial synchrony},
meaning that eventually after an arbitrary long period of asynchrony

\DM{text below seems lengthy to me, and again, a bit judgemental. I would tone
down and say that partially synchronous solutions are vulnerable to "asynchrony
network attacks", that's all.}\sasha{Ok, but I do want to introduce
the leader based approach here} the network communication
becomes synchronous~\footnote{This point in this is usually called global synchronization time (GST)~\cite{}}.
A practical protocol, therefore, has to satisfy safety during
asynchronous periods, and rely on synchrony to satisfy termination.
The common approach for such a protocol is the following: one
pre-defined leader proposes a value and tries to get the other parties
to adopt and then commit this value. 
In case the leader is good and the network is synchronous, all parties
reach agreement and the leader can continue to proposing the next
value.
Otherwise, since it is impossible to distinguish between a bad leader
that intentionally stall the protocol form an asynchronous period,
after some time without progress the leader is replaced with the next
pre-defined leader.
This is done via a \emph{view-change} mechanism that makes sure that
safety is guaranteed despite the leader change.

% \paragraph{eventoul synchrony is not good enouth}
This approach have been used for almost two decades in
data-centers~\cite{} and storage systems~\cite{} \sasha{where else?}
in order to implement a \emph{state machine replication
(SMR)}~\cite{paxosMadeSimple} to replicate and maintain a distributed
shared state on top of crash-prone servers.
However, as pointed out several times in the past~\cite{}, it seems
to be not good enough for a high-stake blockchain system since this
approach has no defence against an adaptive denial of service (DoS)
attacks.
Even if the communication is synchronous, an adaptive adversary
(e.g., any interested and powerful party) can perform a DoS attack on
all leaders, causing the progress to stall forever.


% \paragraph{Asynchronous solutions used to be expensive.}
Asynchronous protocols, on the other hand, are usually
leader-less~\cite{}.
Therefore, they are great candidates for blockchain systems that
wishes to tolerate adaptive DoS attacks.
Unfortunately, these protocols are usually very theoretical, meaning
that they are too complicated and costly for a practical systems.
To the best of our knowledge, Honeybedger~\cite{} is the only
implementation of an asynchronous Agreement protocol.
In its core, Honeybedger uses the byzantine asynchronous Agreement
protocol by Cachin et al.~\cite{} introduced in 2001, which has a
cubic message communication cost.
For almost 20 years no development has been made in reducing its
message communication cost, until recently it was shown in~\cite{} how
to achieve the same result with only a quadratic communication cost.
The protocol in~\cite{} is surprisingly simple. 
It relies on the idea that instead of first choosing a leader and then
letting him try to make progress, which exposes him to DoS attack, we
can let all parties act as leaders and try to make progress
concurrently, and then pick a random leader among them in order to
decide which progress to consider. Since an adversary cannot perform
DoS attack on all leaders concurrently, with high probability we will
pick a leader that made the progress we need.
Therefore, after repeating the above a small number of
times\footnote{They show in~\cite{} that it takes 2 rounds in
expectation to reach agreement}, we get progress with probability 1.
% This paper gives the theoretical basis for our work.

% \paragraph{Optimisitic protocol is the best!}
In the SMR problem, parties are trying to maintain a distributed
shared state.
Each party has a local copy of the state, and the goal is to have the
same state in all parties.
The standard approach to implement an SMR is divided into two
mechanisms: 
First all parties have to agree on the sequence of changes to apply
to the state, and then each party locally executes these changes, one
by one, to its local copy of the state.
To agree on these changes, parties sequentially run instances of
their favorite Agreement protocol.
As mentioned above, using a leader based solutions that is designed
for the partial synchrony model exposes the SMR to DoS attacks and
cannot guarantee progress during asynchronous periods.
On the other hand, while~\cite{} significantly improves the
complexity of asynchronous solutions, it still has a price that we
prefer not to pay when we do not really have to.
In particular, if the network is healthy and the pre-defined leader
follows the protocol, it is possible to reach Agreement with linear
communication cost~\cite{hotstuf?, SBFt?, something else?}.
This leads us to the following question: Is it possible to enjoy both
worlds? Can we design an \emph{Optimistic} protocol that exploit
synchronous periods for great performance but in the same time keep
progress even during long asynchronous periods or adaptive DoS
attacks?


% \paragraph{State transfer is expensive}
To the best of our knowledge, the only attempt to do that so far was
done in a theoretical paper by Cachin at el.~\cite{} in 2005. 
Their basic idea was to run an efficient leader based protocol for a
pre-defined number of Agreement instances or until the parties detect
that progress is stall, and then, before simply replacing the leader
with the next one in line as standard eventual synchronous
solutions do, they run an instance of an asynchronous agreement to
guarantee progress.
Ideally, since the communication cost of the
``expensive'' asynchronous Agreement protocol is amortized in
the best case scenario in which they run a sequence of ``efficient''
leader based Agreement before every asynchronous one, one would
expect to get an amortized linear communication.
However, since parties in their protocol cannot move to the next
instance before learning the decision value of the current one,
they need to make sure that every party gets the decision value of
every instance of the Agreement protocol, which requires a quadratic
message complexity for each instance.
% We describe their protocol in more details in Section~\ref{}.


% \paragraph{we need weaker abstraction}
This is called \emph{state transfer} and it seems to be inherent for
the SMR problem.
However, maybe SMR is simply the wrong abstraction for distributed
ledgers, and we can define a weaker one that on the one
hand has linear optimistic solution, and on the other hand can
guarantee the properties we need.
Recall that an SMR consists of two orthogonal mechanisms: agreeing on
a sequence of operations to apply to the state, and then executing
them.
Now note that in order to guarantee that no two honest parties will
ever end up in a different state, it is enough to agree on the
sequence of operations.
Moreover, we do not need all honest parties to learn this operations
in order to guarantee that no contradicting decision will be ever
made, it is enough that a sufficiently large subset of parties will
do.
If some entity (external or internal) in future will want to learn
these operations, it can simply query all parties and wait for a reply
form a sufficiently large subset of them.
We give a formal definition of our \emph{distributed ledger} in
Section~\ref{}.
\DM{I don't think our definition is different from standard. we have to wait
until we learn that 2f+1 tell us they decide, no?}
\sasha{we are different. we do not build on top of atomic broadcast.
On the one hand we want all parties to halt, but on the other hand we
do not want to pay quadratic communication. In STR the quadratic cost
is inherent due to the state transfer. Therefore, we define a weaker
problem - I can decide not to decide when I know that enough
decided} Intuitively, we relax the standard termination property in the following way: instead requiring that all honest parties eventually decide, we only require that $f+1$
honest do.
In addition, we strengthen the standard termination property by
requiring all honest parties to eventually halt.
Note that while achieving halting with quadratic communication is
trivial by simply forwarding the decision value to all, doing it with
linear cost in the optimistic case is challenging. 

% atomic broadcast is not required for SMR!
% Actually, this weaker definition is exactly what was defined in the
% original paxos~\cite{} paper 

\paragraph{Our contribution.} 
In this paper we present a general framework for optimistic
distributed ledgers.
We first show how to take any leader-based Agreement protocol that
works in the partially synchronous model and turn it into an asynchronous
protocol.
Moreover, we then also show how to use it to implement an
optimistic distributed ledger.
All the framework assumes on the partially synchronous protocols is
that they can be decoupled into a \emph{leader based protocol (LBP)}
and a \emph{view-change} abstractions that satisfy some basic
properties. More details in Section~\ref{}.
The complexity of our general distributed ledger implementation
preserves the complexity of the original protocol in the optimistic
case (synchronous network and correct leader).
And in the worst case (asynchronous network or DoS attack), where the
original protocol stalls, our general protocol adds only a factor of
$n$ compared to the best case.
In particular, as we show in Section~\ref{}, that if we instantiate
our optimistic general solution with a leader
based protocol that has linear communication~\cite{}, then we get an
optimal (not amortized) optimistic solution to distributed ledger
problem:
linear in best case and quadratic in the worst case.


As we mention before, our framework is general.
The properties definition, of the LBP and view-change abstractions,
required by the framework abstracts away all the specific model
assumptions and the specific implementation details made by each of
the eventual synchronous protocol that is instantiated into our
framework.
As a result, for example, our framework can be instantiated with
partially synchronous consensus protocols for the benign case like
Paxos~\cite{} and Raft~\cite{} that assume $n=2f+1$ and at the same
time it can be instantiated with partially synchronous Agreement
protocols for the byzantine case like PBFT~\cite{} and
Zyzzyva~\cite{}.


We implement our framework in C++ and compare its performance to
exciting partially synchronous protocols as well as to the state of
the art asynchronous solution~\cite{}.
In order to achieve optimal performance for the optimistic case we
implement a variant of the linear leader based protocol from
in~\cite{HotStuff} and instantiate it into our framework.
In Section~\ref{}, we show that our optimistic distributed ledger
protocol outperform HoneyBedger~\cite{} in asynchronous and
synchronous networks, and comparable to PBFT~\cite{} and SBFT~\cite{}
in synchronous networks.
Moreover we show, that under adaptive DoS attacks our protocol
performs like in the asynchronous case, whereas PBFT and SBFT stall.

% \paragraph{Summary of contribution}
In summary, our paper makes the following contribution:

\begin{itemize}
  
  \item We defines a general framework, based on two clean
  abstractions, to turn any Agreement solution in the eventually
  synchronous model to an asynchronous protocol.
  
  \item The framework abstracts away all specific model assumptions
  and implementation details made by each of the eventually
  synchronous solutions.
  
  \item When instantiated with a partially synchronous consensus
  protocols for the benign case (e.g., Paxos~\cite{} and
  Raft~\cite{}), the framework yields the first asymptotically optimal
  asynchronous consensus solution for the benign case.
  
 \item When instantiated with a linear partially synchronous
 Agreement protocol for the byzantine case, the framework yields the
 first asynchronous optimistic distributed ledger implementation that
 can tolerate adaptive DoS attacks, and has linear communication in
 the best case and quadratic communication in the worst case.
 
 \item We implement our framework in C++ and instantiate it with our
 implementation of a variant of the linear leader based protocol from
in~\cite{HotStuff}.

 \item We compare our implementation's performance to exciting
 partially synchronous protocols as well as to the state of the art
 asynchronous solution~\cite{}.
   
  
\end{itemize} 

The rest of the paper is organized as follows: \ldots\ldots\ldots





==> model.tex <==
\section{Model and Problem Definitions}

\subsection{System Model}
\label{sec:model}


We consider a peer to peer system with $n$ parties, $f<n$ of which may
fail.
We say that a party is \emph{faulty} if it fails at any time during an
execution of a protocol.
Otherwise, we say it is \emph{correct}.
In a peer to peer system every pair of parties is connected with a
\emph{communication link}.
A message sent on a link between two correct parties is guaranteed to
be delivered, whereas a message from or to a faulty party might be
lost.
A link between two correct parties is \emph{asynchronous} if the
delivery of a message may take arbitrary long time, whereas
a link between two correct parties is \emph{synchronous} if there is
known bound~\footnote{Even if the bound is unknown, parties may learn it with standard
techniques.} $\Delta$ for message deliveries.
In \emph{asynchronous network periods} all links among correct parties
are asynchronous, whereas during \emph{synchronous network periods}
all such links are synchronous.
We measure the theoretical \emph{communication cost} of a protocol by
the total number of messages sent on links among correct parties. 


\DM{It seems that we have two "stories":
(i) we work in a pure asynchronous settings, but aim for optimistic performance
comparable to practical solutions in the pratial synchrony model. (ii) we work
in a new model called "Weak Adaptive ..." (WAANP). This model is incomparable
with partial synchrony. On one hand, it doesn't have
GST, therefore it is stronger. On the other hand, the asynchrony is constrained
(to one party). We can have both "stories". But
I am not sure I am on board with using WAANP as a tool for
demonstrating a concrete scenario that do not make progress in the partial-synchrony model before GST. No one
claims progress before GST anyway!}
\sasha{Just a  way to formalize a possible attack on the protocol.
Originally, GST has nothing to do with malicious adversary. It
captures the nature of a real wide area (not byzantine) network. In
blockchain, we deal with new evil, and I think WAANP is one way to
model it. In real system with evil adversary a GST event might never
happen}
\DM{As for HB, it is a fully asynchronous protocol, it is guaranteed
to make progress even in a stronger setting than WAANP. So I don't
understand what we are saying before.}\sasha{Where before?} 
To demonstrate the weakness of existing partially synchronous protocols, we define the notion of \emph{weak adaptive asynchrony
network period}.
In such periods, there is one unique party, at any given time, who's 
links are asynchronous while all other links are synchronous.
This one unique party can be changed arbitrary during the period.
This definition captures the adaptive DoS attacks mentioned in the
Introduction.
To the best of our knowledge, Honeybedger~\cite{} is the only
existing Agreement practical implementation that can guarantee
progress during weak adaptive asynchrony network periods.
Moreover, as we explain in more details and demonstrate below, leader
based protocol are inherently unable to tolerate such network periods.

\DM{Again, as per above: We only compare (optimistic) performance,
right?}\sasha{With PBFT-like prtocols, yes. But with Honeybedger we
compare both synchronous and asynchronous periods. } In order
to be able compare our framework with existing practical solutions we use the standard \emph{partially synchronous} model~\cite{}.
In this model, there is an unknown point in every execution, called
\emph{global stabilization time (GST)}, that divides the execution
into two network periods: Before the GST the network is asynchronous
and after the GST the network is synchronous.

As mentioned in the Introduction and explained in more details below,
our general framework abstracts away specific model assumptions and
implementation details into several primitives: \emph{Leader based
protocol (LBP)}, \emph{view-change}. \emph{leader-election},
\emph{barrier}, and \emph{view-change-trigger} \sasha{TODO: find
better name}.
In Section~\ref{}, we define the properties of these primitives and
require that any partially synchronous protocol that is instantiated
into our framework satisfies them during asynchronous periods.
To satisfy these properties, each protocol may have different
model assumptions.
For example, the relation between $f$ and $n$, and the type of
failures that may occur (e.g., crash and byzantine).
Our framework inherent the specific assumptions made by
each of the partially synchronous protocol it instantiated with, but
adds nothing to it.
In other words, whatever assumptions are made by the instantiated
protocol in order to satisfy the primitives' properties, are
exactly the assumption under which our framework operate.





% Define honest ot be a player that follow the protocol. 




% We do not need to increasing timeouts like PBFT like solutions because
% we have the barrier for synchronization.




==> modelBeforePLDImodel.tex.tex <==
\section{Model and Problem Definitions}

\subsection{System Model}
\label{sec:model}


We consider a system with $n$ parties, $f<n$ of which may
fail.
We say that a party is \emph{faulty} if it fails at any time during an
execution of a protocol.
Otherwise, we say it is \emph{correct}.
Every pair of parties is connected with a
reliable \emph{communication link}.


\subsubsection*{Synchrony, Asynchrony and Partial Synchrony}
\ittai{I will re-write this:}

\begin{comment}
A message sent on a link between two correct parties is guaranteed to
be delivered, whereas a message from or to a faulty party might be
lost.
A link between two correct parties is \emph{asynchronous} if the
delivery of a message may take arbitrary long time, whereas
a link between two correct parties is \emph{synchronous} if there is
known bound~\footnote{Even if the bound is unknown, parties may learn it with standard
techniques.} $\Delta$ for message deliveries.
In \emph{asynchronous network periods} all links among correct parties
are asynchronous, whereas during \emph{synchronous network periods}
all such links are synchronous.
We measure the theoretical \emph{communication cost} of a protocol by
the total number of messages sent on links among correct parties. 

\end{comment}

\subsubsection*{The problem with Partial Synchrony}
\ittai{I like the WAAP model! will shorten this a bit}
To demonstrate the weakness of existing partially synchronous protocols, we define the notion of \emph{weak adaptive asynchrony
network period}.
\begin{comment}
In such periods, there is one unique party, at any given time, who's 
links are asynchronous while all other links are synchronous.
This one unique party can be changed arbitrary during the period.
This definition captures the adaptive DoS attacks mentioned in the
Introduction.
To the best of our knowledge, Honeybedger~\cite{} is the only
existing Agreement practical implementation that can guarantee
progress during weak adaptive asynchrony network periods.
Moreover, as we explain in more details and demonstrate below, leader
based protocol are inherently unable to tolerate such network periods.
\end{comment}






% Define honest ot be a player that follow the protocol. 




% We do not need to increasing timeouts like PBFT like solutions because
% we have the barrier for synchronization.




==> provableFramework.tex <==
% Next section Framework for Distributed ledger
% 
% Next section: Optimistic ledger Implementation


\section{Extended Framework For Distributed Ledgers}\label{subsec:practical}



% This is important because we want parties to be able to jump forward
% to higher views and slots.
Recall that by Halting, all honest parties in a given slot eventually
halt.
But by Noticeable termination, some honest parties may never decide,
and thus never move forward to the next slot.
Therefore, honest parties that do move must be able to convince slow
ones that enough parties have decided and it is safe to move forward.
To this end, in order to be able to generalize the optimistic (single
shoot) Agreement into an optimistic distributed ledger, we need to
slightly strengthen the properties required by the primitives we use
in order to allow parties to prove their outputs.
Note that in case of crash failures we get this for free, while in the
byzantine failure case, some cryptography is required. 

For the \LBP, we extend the \emph{approve} API to return (in addition
to state and value) a proof a $\sigma$, and assume a known to all
function \emph{doneVerify} that gets an instance identification and a
proof, and returns either \emph{true} or \emph{false}.
We call this extension \PLBP. 
To fit for framework, a \PLBP\ instance with identification $id$
must satisfy the following properties in every alternate executions:

  
  \begin{itemize}
    
    \item \textbf{pLBP-Termination:} If the leader of the instance
    is honest, all honest parties invoke \emph{approve}, and no honest
   party invokes \emph{abandon}, then (1) the leader's propose
   invocation eventually returns, and (2) every honest parties returns
   a proof $\sigma$ s.t.\ \emph{doneVerify}$(id,\sigma)$ =
   \emph{true}.
    
    \item \textbf{pLBP-Completeness:} If a propose invocation by an
    honest leader returns, then at least $f+1$ honest parties return a
    proof $\sigma$ s.t.\ \emph{doneVerify}$(id,\sigma)$ = \emph{true}.
    
    \item \textbf{pLBP-Provability} If some party produces a proof
    $\sigma$ s.t.\ \emph{doneVerify}$(id,\sigma)$ = \emph{true}, then
    at least $f+1$ honest parties return \emph{value} $v \neq \bot$.
    
    \item \textbf{pLBP-Abandonment:} If an honest party invokes
    \emph{abandon()}, then its \emph{approve} operation immediately
    returns.
  
  \end{itemize}
  
As for the \emph{view-change trigger} abstraction, we extend the
\emph{trigger-sync()} API to return a proof $\sigma$, and assume a
known to all function \emph{triggerVerify} that gets an instance
identification and a proof, and returns either \emph{true} or
\emph{false}.
We call this extension \emph{Provable-trigger}, and assume the
following properties:

\begin{definition}[Provable-trigger]

An implementation of a Provable-barrier abstraction with
identification $id$ must satisfy the following properties:

\begin{itemize}
  
  \item \textbf{pT-Validity:} If a trigger-sync() invocations by an
  honest party returns a proof $\sigma$, then
  \emph{barrierVerify}$(id,\sigma)$ = \emph{true}.
  
  \item \textbf{pB-Provability:} If some party produces a proof
    $\sigma$ s.t.\  \emph{barrierVerify}$(id,\sigma)$ = \emph{true},
    then some honest party previously invoked trigger().
  
  \item \textbf{pB-Termination:} If $f+1$ honest parties invoke
  trigger() then all trigger-sync() invocations by honest parties
  eventually return.

\end{itemize}

\end{definition}


For the Leader-election abstraction, we extend the \elect API
to return a proof $\sigma$ for the elected leader, and assume a known
to all function \emph{leaderVerify} that gets an instance
identification, a leader, and a proof, and returns either \emph{true}
or \emph{false}.
We call this extension Provable-leader-election, and assume the
following properties:


\begin{definition}[Provable-leader-election]

An implementation of a Provable-leader-election abstraction with
identification $id$ must satisfy the following properties:

\begin{itemize}
  
  \item \textbf{pL-Termination:} If $f+1$ honest parties invoke
  \elect, then all invocations by honest parties eventually
  return a leader $l$ and a proof $\sigma$ s.t.\
  \emph{leaderVerify}$(id,l,\sigma)$ = \emph{true}.
  
  \item \textbf{pL-Agreement:} All invocations of \elect by honest
  parties return the same party.
  
  \item \textbf{pL-Validity:} If an invocation of \elect by an
  honest party returns, it returns a leader $p$ with probability $1 /
  |\Pi|$ for every $p \in \Pi$.
  
  \item \textbf{pL-Unpredictability:} The probability of the adversary
  to predict the returned leader of an \elect invocation by an
  honest party before any honest party invokes \elect is at most $1
  / |\Pi|$.
  
  \item \textbf{pL-Provability:} If some party produces a proof
    $\sigma$ s.t.\  \emph{leaderVerify}$(id,l,\sigma)$ =
    \emph{true}, then no \elect invocation by an honest party
    return $leader \neq l$.
  
\end{itemize}


\end{definition}











==> singleShotProof.tex <==

\section{Single-Shot Agreement Correctness Proof (Section 5.1)}
\label{sec:proof}

We prove that Algorithm~\ref{alg:AS} satisfies 
Agreement, Termination, Validity, and Fairness properties
in the asynchronous communication model.
We start by proving the Agreement and Validity properties.


\begin{observation}
\label{obs:compose}

The chosen LBV instances in Algorithm~\ref{alg:AS} form a properly
composed execution.

\end{observation}

\begin{lemma}
\label{claim:AS:V_A}

Algorithm~\ref{alg:AS} satisfy the \emph{Validity} and
\emph{Agreement}.

\end{lemma}

\begin{proof}


By the code, correct parties only decide on values returned from a
\vc method invoked on one of the chosen instances.
Therefore, by Observation~\ref{obs:compose}, the Validity and Agreement
properties follow from the Safety properties required by the LBV
abstraction.

\end{proof}


\noindent We now prove that Algorithm~\ref{alg:AS} satisfies
Termination.
We start by showing that no honest party is stuck forever in a
wave.

\begin{claim}
\label{claim:AS:ready}

Consider a wave $k \geq 1$ that all correct parties start, then at
least one \barriersync invocation by a correct party eventually
returns.

\end{claim}

\begin{proof}

Assume by way of contradiction that no \barriersync()
invocations by correct party eventually returns in wave $k$.
Thus, no correct party ever invoke \vc in wave $k$.
Therefore, since all correct parties invoke \propose in all
LBV instances in wave $k$,
we get by the Engage-Termination property that all
\emph{propose} invocation by correct parties eventually return, and
thus all correct parties eventually send $\textsc{engage-done}$
messages to all correct leaders.
Hence, all correct leaders eventually get $n-f$ $\textsc{engage-done}$
messages, and thus eventually invoke \barrierready.
The contradiction follows from the B-Termination property.


\end{proof}


\begin{claim}
\label{claim:AS:view}

For every wave $k \geq 1$, if all correct parties start wave $k$, then
all correct parties eventually complete wave $k$.

\end{claim}

\begin{proof}

By Claim~\ref{claim:AS:ready}, some \barriersync
invocation by a correct party eventually returns in wave $k$.
Thus, by the B-Agreement property, all \barriersync
invocations by correct parties eventually return in wave $k$, and
thus all correct parties eventually invoke \elect in wave $k$.
By the L-Termination property, all \elect invocations by
correct parties eventually return in wave $k$.
Therefore, the Claim follows from the Wedge\&Exchange-Termination
property.

\end{proof}

\noindent The next corollary follows by inductively applying
Claim~\ref{claim:AS:view}.

\begin{corollary}
\label{col:viewcomplete}

For every $k \geq 1$, all parties eventually complete wave $k$ in
Algorithm~\ref{alg:AS}.

\end{corollary}

\noindent For the rest of the proof we say that an LBV instance is
\emph{completed} if at least $f+1$ \propose innovations by correct
parties previously returned.
We next bound the probability to choose a leader of a completed LBV
instance.

\begin{claim}
\label{claim:AS:leader}

For every wave $k \geq 1$, at least $f+1$ LBV instances with correct
leaders are completed before some correct party invokes \elect.

\end{claim}

\begin{proof}

Consider some correct party that invokes \elect at wave
$k$.
By the code, its \barriersync invocation was previously
returned, and thus by the B-Coordination property, at least $f+1$
correct parties previously invoked \barrierready.
Therefore, at least $f+1$ correct parties
received $n-f$ $\textsc{engage-done}$ messages, at least
$f+1$ of which are from correct parties.
Since correct parties send $\textsc{engage-done}$ messages to party
$p_j$ only after their \propose invocation in the LBV instance in
which $p_j$ acts as leader returns, at least $f+1$ LBV
instances with correct leaders are completed before some correct party
invokes \elect.

\end{proof}

\begin{claim}
\label{AS:probability}

Consider a wave $k \geq 1$ that all parties start, the probability for
all correct parties to decide at wave $k$ is at least $\frac{f+1}{n}$.

\end{claim}

\begin{proof}

By Corollary~\ref{col:viewcomplete}, all correct parties invoke
\elect in view $k$ and, by the L-Agreement property, all
invocations return the same leader.
By Claim~\ref{claim:AS:leader}, at least $f+1$ LBV instances are
completed before some correct party invokes \elect at view $k$.
Therefore, by the L-Validity and L-Unpredictability properties, we get
that the probability to choose a leader of a completed LBV instance is
at least is $\frac{f+1}{n}$.
By the Completeness property of the LBV abstraction, if a completed
LBV instance is chosen, then no \vc invocation by correct party
returns $v= \bot$.
Therefore, by the code, all correct parties decide at the end of wave
$k$ with probability $\frac{f+1}{n}$. 


% Therefore, by the Completeness property of the LBV abstraction, the
% probability that at least $f+1$ honest parties return \emph{value} $v
% \neq \bot$ at view $k$ is $p$.
% Hence, by Claim~\ref{col:viewcomplete} and the VC-Causality property,
% all $VC$ invocations by honest parties return a value $v \neq \bot$
% at view $k$ with a probability $p$, and thus all honest parties decide
% at the end of view $k$ with a probability $p$.

\end{proof}

\begin{lemma}

Algorithm~\ref{alg:AS} satisfies Termination. 

\end{lemma}

\begin{proof}

By Corollary~\ref{col:viewcomplete}, correct parties are never
stuck indefinitely in any view, and thus all honest parties eventually start
all views.
Therefore, by Claim~\ref{AS:probability}, all honest parties
eventually decide with probability 1.
Moreover, the expected number of views after which all correct party decide
is $\frac{n}{f+1}$.

\end{proof}


\begin{lemma}

Algorithm~\ref{alg:AS} satisfies Fairness. 

\end{lemma}

\begin{proof}


By the Completeness property of the LBV abstraction, if a completed
instance is chosen, than all correct parties decide at the end of
the wave. 
By Claim~\ref{claim:AS:leader}, for every wave $k \geq 1$, at least
$f+1$ LBV instances with correct leaders are completed before a
unique instance is chosen in the wave.
Therefore, even if all LBV instances with faulty parties have been
completed as well, the probability to decide on value proposed by a
correct party is at least $1/2$. Moreover, during synchronous periods,
all instances with correct parties complete with equal probability,
and thus by the L-validity, all correct parties have an equal
probability for their values to be chosen.


\end{proof}

==> sync.tex <==
\section{Synchronous }

Recent works embrace leader-based regime in synchronous solutions in order to
speed up the common mode. In the synchronous model, there is a known upper bound
$\Delta$ on transmission delays among honest parties.
Leader-based synchronous Agreement was pioneered by Abraham et al~\cite{FC19}, a lock-step protocol
with $4\Delta$ (?) common-mode latency. Dfinty Consensus~\cite{dfinty, our notes
explaining it} removed the need for lock-step. Sync HotStuff~\cite{sync-hs}
further improves on Dfinty by reducing the common-mode latency to $2\Delta$. 
In all these works, a rushing adversary may cause $O(n\Delta)$ latency to
decision.

By employing our framework in the synchronous setting, we can thwart a rushing
adversary and achieve expected $6\Delta$ (?) latency to decision.

We introduce a cubic protocol. We then discuss two
improvements. First, similar to the asynchronous setting, one can
employ optimism, alternating between a single-leader (optimistic) phase and a
multi-leader (pessimistic) phase. Second, we can alternate between synchronous
and asynchronous leader protocols in between view-changes.

\begin{algorithm}
\caption{Synchronous Agreement: protocol for party $p_i$.} 
\begin{algorithmic}[1]

\Upon{\emph{SYN-propose(S)} or receiving any other propose message}
 
\State $state \gets S$
\State $view \gets 1$
\While {true}
	\State $id \gets view$
	\State $\lr{state, value\textcolor{gray}{, leader,
	leaderProof, doneProof}} \gets tryPessimistic(id, state)$
	\State $\lr{state,value} \gets VC_{id}(state,value)$
	
	\If{$value \neq \bot$ }
		\State \textbf{decide} value
	\EndIf
	\State $view \gets view+1$ 
\EndWhile
\EndUpon

\Statex
\Procedure{tryPessimistic}{$id, state$}

 	\State invoke $propose_{\lr{id,p_i}}(state)$ \Comment{non-blocking}
	
	\ForAll{$p_j=p_1,\ldots,p_n$}
		\State invoke $approve_{\lr{id,p_j}}(state)$ \Comment{non-blocking}
	\EndFor

	\State wait $3\Delta$ \Comment{one $\Delta$ for all instances to start,
two to decide}
	\State send $blame_j$ for every $j$ without a decision
	\State wait another $\Delta$
	\State for every $j$ with $f+1$ blames, stop approving in instance $j$
	
	\State $\lr{leader \textcolor{gray}{,leaderProof}} \gets $
	\emph{$elect_{id}()$}
	
	\State let $\lr{state',value'\textcolor{gray}{,doneProof}}$ be the
	return value of $approve_{\lr{id,leader}}(state)$
	
	\State \textbf{return} $\lr{state', value'\textcolor{gray}{, leader,
	leaderProof, doneProof}}$
	
 	
\EndProcedure

\Statex 

\Upon{\emph{propose}$_{\lr{id,p_i}}$ returns \textsc{Ack}}
	\State invoke $\emph{ready}_{id}()$
\EndUpon

\end{algorithmic}
\label{alg:SYN}
\end{algorithm}


